Towards Privacy-, Budget-, and Deadline-Aware Service Optimization for Large Medical Image Processing across Hybrid Clouds

Efficiently processing medical images, such as whole slide images in digital pathology, is essential for timely diagnosing high-risk diseases. However, this demands advanced computing infrastructure, e.g., GPU servers for deep learning inferencing, and local processing is time-consuming and costly. Besides, privacy concerns further complicate the employment of remote cloud infrastructures. While previous research has explored privacy and security-aware workflow scheduling in hybrid clouds for distributed processing, privacy-preserving data splitting, optimizing the service allocation of outsourcing computation on split data to the cloud, and privacy evaluation for large medical images still need to be addressed. This study focuses on tailoring a virtual infrastructure within a hybrid cloud environment and scheduling the image processing services while preserving privacy. We aim to minimize the use of untrusted nodes, lower monetary costs, and reduce execution time under privacy, budget, and deadline requirements. We consider a two-phase solution and develop 1) a privacy-preserving data splitting algorithm and 2) a greedy Pareto front-based algorithm for optimizing the service allocation. We conducted experiments with real and simulated data to validate and compare our method with a baseline. The results show that our privacy mechanism design outperforms the baseline regarding the average lower band on individual privacy and information gain for privacy evaluation. In addition, our approach can obtain various Pareto optimal-based allocations with users' preferences on the maximum number of untrusted nodes, budget, and time threshold. Our solutions often dominate the baseline's solution and are superior on a tight budget. Specifically, our approach has been ahead of baseline, up to 85.2% and 6.8% in terms of the total financial and time costs, respectively.

==> Tables/table1.tex <==
\begin{table}[!thb]
    \centering
    \caption{Summary of notations}\label{tab:notations}
    \begin{tabularx}{0.48\textwidth}{lX}
        \toprule
        \textbf{Notation} & \textbf{Description} \\
        \midrule
        $\mathcal{A}$ & data (e.g., medical image) processing application \\
        $\mathcal{M}$ & a set of microservices, $\mathcal{M}=\{m_{\text{splt}}, m_{\text{inf}}, m_{\text{aggr}}\}$ \\
        $m_{\text{splt}}$ & data splitting function for the application\\
        $m_{\text{inf}}$ & inference function of the application \\
        $m_{\text{aggr}}$ & aggregation function of the application \\
        $\epsilon$ & a set of data streams\\
        $\mathcal{D}$ & source data set, e.g., WSIs \\  
        $S_{\text{trust}}$ & a trusted server (zone) \\
        $\mathcal{I}$ & a provisioned infrastructure, $\mathcal{I} = \mathcal{I}_{c}\cup \mathcal{I}_{-c}$ \\
        $\mathcal{N}_I$ & the number of $\mathcal{I}$, $\mathcal{N}_I=\mathcal{N}_h + \mathcal{N}_c$ \\
        $\mathcal{N}_h, \mathcal{N}_c$ & the number of honest and corrupted nodes \\
        % $req$ & a set of user requirements \\
        % $\mathcal{I}^{u}_{1}, ..., \mathcal{I}^{u}_{\mathcal{N}_{\mathcal{I}^u}}$ & a set of $\mathcal{N}_{\mathcal{I}^u}$ infrastructures from universities \\
        % $\mathcal{I}^{c}_{1}, ..., \mathcal{I}^{c}_{\mathcal{N}_{\mathcal{I}^c}}$ & a set of $\mathcal{N}_{\mathcal{I}^c}$ infrastructures from CSPs \\
        $\mathcal{I}_{1}, ..., \mathcal{I}_{K}$ & a set of Cloud instances over $\mathcal{I}$\\
        % $f$ & parallel code fragment that can be reusable over $\mathcal{I}$ \\
        % $1-f$ & sequential code fragment over $S_{\text{trust}}$ \\
        $T^{(k)}_{\text{comm.}}$ & communication time between $S_{\text{trust}}$ and the target $\mathcal{I}_{k}$\\
        $T^{(k)}_{\text{compt.}}$ & computational cost over $\mathcal{I}_{k}$\\
        $p_k$ & unit price of $\mathcal{I}_{k}$ (i.e., US dollar (\$) per hour)\\
        $D$ & image tiles (or patches) data set from $\mathcal{D}$ \\
        % $D^P$ & perturbed data from $D$ \\
        % $D^r$ & reconstructed data from the perturbed data $D^p$ \\
        $H(\cdot)$ & the Shannon's information entropy \\
        $A_x$ & distribution or coordinates system of $D$ over a grid \\
        $D_{e}$ & encoded data sets, $D_{e}=\{D_{e,1}, ..., D_{e,K}\}$ \\
        $\mathcal{G}$ & the network graph over a provisioned infrastructure \\
        % , where $\mathcal{G}=(\mathcal{V}, \mathcal{E})$ \\
        $G$ & the graph extracted from $D$ \\
        % , where $G=(V, E)$ \\
        $\chi(\mathcal{D})$ & the chromatic number of data set $\mathcal{D}$ \\
        $\theta_k$ & workload $k$, $\theta_k = (m_{\text{inf}}, D_{e,k})$ \\
        $\Theta$ & workloads of $\mathcal{A}$, $\Theta = \{\theta_1, ..., \theta_l\}$\\ 
        $x_k$ & a boolean value. 1, if $\theta_k$ maps to $\mathcal{I}_{k}$; 0, otherwise. \\
        $f_1$ & the total number of distributed processing nodes \\
        $f_2$ & the monetary cost of $\mathcal{A}$ \\
        $f_3$ & the maximum completion time of $\mathcal{A}$ \\
        % $T_{compt.}$ & benchmark $T_{compt.}(\Theta, \mathcal{I}_{base})$ \\
        % $T^{\text{berk}}_{\text{compt.}}$ & a benchmark tested and calculated over $\mathcal{I}$\\
        $\mathbf{x}_{\text{pareto}}$ & the Pareto optimal solution \\
        % $\mathbf{x}_{\text{base}}$ & the baseline solution \\
        \textit{Pfdata} & the set of Pareto optimal solutions \\
        \bottomrule
    \end{tabularx}   
\end{table}

==> Tables/table4.tex <==
% \begin{table*}[!t]
%     \caption{A short description of the split data sets implemented by Algorithm~\ref{alg: privacy method}. We presented the total number of patches and its size from each sub data set.}
%     \label{tab: dataset}
%     \centering  
%     \begin{tabular}{ccccccccccccc}
%     \toprule
%         \multirow{2}*{\textbf{No}} & \multirow{2}*{\textbf{Total patches}} & \multirow{2}*{\textbf{$\chi(\mathcal{D})$}}
%         & \multicolumn{2}{c}{\textbf{$D_{1,e}$}} & \multicolumn{2}{c}{\textbf{$D_{2,e}$}} & \multicolumn{2}{c}{\textbf{$D_{3,e}$}} & \multicolumn{2}{c}{\textbf{$D_{4,e}$}} & \multicolumn{2}{c}{\textbf{$D_{5,e}$}}\\ \cline{4-13}
%         \textbf{} & \textbf{ } & \textbf{ } & \textbf{Patches} & \textbf{Size} & \textbf{Patches} & \textbf{Size} & \textbf{Patches} & \textbf{Size} & \textbf{Patches} & \textbf{Size} & \textbf{Patches} & \textbf{Size}\\
%         \midrule
        
%         I & 7740 & 5 & 2873 & 379MB & 2881 & 383,5MB & 1497 & 201,3MB & 479 & 64,9MB & 10 & 1,2MB\\
%         II & 11637 & 5 & 4279 & 547,5MB & 4279 & 549,9MB & 2262 & 290,9MB & 800 & 104MB & 17 & 2,2MB \\
%         III & 20589 & 5 & 7606 & 895,9MB & 7623 & 898,2MB & 3978 & 477,7MB & 1358 & 164,1MB & 24 & 2,9MB \\
%         IV & 20467 & 5 & 7508 & 970,8MB & 7532 & 974,2MB & 3994 & 518,2MB & 1407 & 182,4MB & 28 & 3,7MB \\
%         V & 4040 & 5 & 1539 & 189,3MB & 1515 & 187,5MB & 746 & 92,3MB & 245 & 30,5MB & 4 & 455KB \\
%         VI & 13002 & 5 & 4892 & 555,9MB & 4833 & 556,4MB & 2456 & 285,2MB & 802 & 95,2MB & 19 & 2,2MB \\
%         VII & 23136 & 5 & 8527 & 890,3MB & 8487 & 890,8MB & 4526 & 481,8MB & 1565 & 171MB & 31 & 3,8MB \\
%         VIII & 40412 & 5 & 14784 & 1,52GB & 14842 & 1,53GB & 7901 & 817,5MB & 2818 & 295,2 MB & 67 & 7,2MB \\
%         IX & 41299 & 5 & 15175 & 1,48GB & 15187 & 1,49GB & 8116 & 811,7MB & 2767 & 275MB & 54& 5,3MB \\
%         X & 30952 & 5 & 11481 & 1,09GB & 11436 & 1,09GB & 5926 & 578,8MB & 2051 & 200,4MB & 58 & 5,7MB \\
%     \bottomrule
%     \end{tabular}
% \end{table*}


==> Tables/table5.tex <==
\begin{table}[!htb]
    \caption{The results of average information gain and resistance attacks of the proposed algorithm. The column AIG represents the average information gain for coordinates. The columns NI and ICA represent naive inference and independent component analysis, respectively.}
    \label{tab:privacyres}
    \centering  
    \begin{tabular}{ccccc}
    \toprule
        \multirow{2}*{\textbf{Data}} & \multicolumn{2}{c}{\textbf{NI}} & \multicolumn{2}{c}{\textbf{AIG}} \\ \cline{2-5}
        \textbf{} & \textbf{$x\_coord$} & \textbf{$y\_coord$} & \textbf{$x\_coord$} & \textbf{$y\_coord$} \\
        \midrule
        A7-A0D9 & 59160.341 & 5559.772 & 3.862 & 4.516  \\
        A7-A3IZ & 12012.008 & 6900.9 & 4.424 & 4.672  \\
        E9-A1N3 & 15279.559 & 7943.6 & 4.651 & 5.003  \\
        AC-A2FB & 22384.322 & 5660.518 & 4.359 & 5.357  \\
        AC-A2FE & 9216.605 & 5043.145 & 3.669 & 4.084  \\
        B6-A0IJ & 33550.891 & 7458.903 & 3.534 & 4.984  \\
        E9-A1NE & 14655.884 & 13999.84 & 4.846 & 4.736   \\
        E9-A1QZ & 20810.58 & 16748.037 & 5.345 & 4.999  \\
        E9-A1R3 & 27007.924 & 4111.707 & 4.834 & 5.307  \\
        E9-A1R4 & 17934.664 & 15893.799 & 5.129 & 4.816   \\
    \bottomrule
    \end{tabular}
\end{table}



==> Tables/table6.tex <==
\begin{table*}[!ht]
    \centering
    \caption{The specification of GPU cloud virtual machines.}
    \begin{tabular}{cccccccc}
     \toprule
         \textbf{Node} & \textbf{GPUs per Server} & \textbf{vCPUs} & \textbf{RAM (GB)} & \textbf{Local Storage (GB)} & \textbf{Location} & \textbf{Price (/Hour)} & \textbf{RPerf} \\ 
         \midrule
         i & Tesla T4 16GB $\times$ 1  & 4 & 7.8  & 40 & Amsterdam, Netherlands& 0 & 1/2.23 \\ 
         ii & Tesla T4 16GB $\times$ 1  & 4 & 7.8  & 40 & Amsterdam, Netherlands& 0 & 1/2.23 \\ 
         iii & RTX 3090 24GB $\times$ 1 & 48 & 125 & 40 & Valencia, Spain & 0 & 1 \\
         iv & RTX 3090 24GB $\times$ 1 & 48 & 125 & 40 & Stavanger, Norway & 0 & 1 \\
         v & A100 PCIE 80GB  & 2 & 4 & 100 & Illinois, USA & \$2.15  & 1/1.55\\ 
         vi & A100 PCIE 40GB  & 2 & 4 & 100 & Illinois, USA & \$2.01 & 1/1.55\\ 
         vii & V100 PCIE 16GB & 2 & 4 & 100 & Illinois, USA & \$0.81 & 1/1.62 \\ 
         viii & RTX A6000 48GB & 2 & 4 & 100 & New York, USA & \$1.27 & 1/0.9 \\
         ix & RTX A6000 48GB & 2 & 4 & 100 & Illinois, USA & \$1.27 & 1/0.9 \\
         x & RTX A5000 24GB & 2 & 4 & 100 & New York, USA & \$0.78 & 1/1.22 \\
         xi & RTX A5000 24GB & 2 & 4 & 100 & Illinois, USA & \$0.78 & 1/1.22 \\
         xii & RTX A5000 24GB & 2 & 4 & 100 & Nevada, USA & \$0.78 & 1/1.22 \\
         xiii & RTX A4000 16GB & 2 & 4 & 100 & New York, USA & \$0.63 & 1/1.57 \\
         xiv & RTX A4000 16GB & 2 & 4 & 100 & Illinois, USA & \$0.63 & 1/1.57 \\
         xv & A40 48GB & 2 & 4 & 100 & New York, USA & \$1.27 & 1/0.93 \\
         xvi & A40 48GB & 2 & 4 & 100 & Illinois, USA & \$1.27 & 1/0.93 \\
         xvii & A40 48GB & 2 & 4 & 100 & Nedada, USA & \$1.27 & 1/0.93 \\
         xviii & QUADRO RTX 5000 6GB & 2 & 4 & 100 & New York, USA & \$0.59 & 1/1.78 \\
         xix & QUADRO RTX 5000 6GB & 2 & 4 & 100 & Illinois, USA & \$0.59 & 1/1.78 \\
         xx & QUADRO RTX 5000 6GB & 2 & 4 & 100 & Nevada, USA & \$0.59 & 1/1.78 \\
         xxi & QUADRO RTX 4000 8GB & 2 & 4 & 100 & New York, USA & \$0.28 & 1/2.38 \\
         xxii & QUADRO RTX 4000 8GB & 2 & 4 & 100 & Illinois, USA & \$0.28 & 1/2.38 \\
         xxiii & QUADRO RTX 4000 8GB & 2 & 4 & 100 & Nevada, USA & \$0.28 & 1/2.38 \\
         xxiv & RTX 3060 TI 8GB & 4 & 12 & 80 & Norway & \$0.34 & 1/1.74 \\
         xxv & RTX 3090 24GB & 4 & 24 & 80 & Norway & \$0.59 & 1 \\
         xxvi & RTX 3090 24GB & 4 & 24 & 80 & Iceland & \$0.59 & 1 \\
         xxvii & RTX 3080 10GB & 4 & 12 & 80 & Norway & \$0.50 & 1/1.14 \\
         xxviii & RTX 3080 10GB & 4 & 12 & 80 & Iceland & \$0.50 & 1/1.14 \\
         xxix & V100 PCIE 16GB & 8 & 120 & 900 & India & \$1.07 & 1/1.62 \\
         \bottomrule
    \end{tabular}
    \label{tab: infracloud}
\end{table*}

==> Tables/table7.tex <==
\begin{table}[!t]
    \centering
    \caption{Comparisons our approach with two baselines.}
    \label{tab: my_cmpr}
    \begin{tabular}{cccc}
    \toprule
       \textbf{Method}  & \textbf{No} ($f_1$) & \textbf{Cost} ($f_2$) & \textbf{Time} ($f_3$) \\
       \midrule
       Time greedy  & 5 (+) & 0.173059 (-) & 169.23 (+) \\
       Cost greedy  & 5 (+) & 0.001878 (+) & 419.30 (-) \\
       Our approach & 6 (+) & 0.032359 (+) & 187.91 (+) \\
    \bottomrule
    \end{tabular}  
\end{table}

% \begin{table*}[!t]
%     \centering
%     \caption{Comparisons our approach with two baselines.}
%     \label{tab: my_cmpr}
%     \begin{tabular}{ccccccc}
%     \toprule
%        \textbf{Method}  & \textbf{No} ($f_1$) & \textbf{Cost} ($f_2$) & \textbf{Time} ($f_3$) & $f_1$ \textbf{violation rate} & $f_2$ \textbf{violation rate}& $f_3$ \textbf{violation rate}\\
%        \midrule
%        Time greedy  & 5 & 0.173059 & 169.23 & 0 & &\\
%        Cost greedy  & 5 & 0.001878  & 419.30 & 0 && \\
%        Our approach & 6 & 0.032359 & 187.91 &0 &&\\
%     \bottomrule
%     \end{tabular}  
% \end{table*}
